On-the-fly Resource-Aware Model Aggregation for Federated Learning in Heterogeneous Edge

Edge computing has revolutionized the world of mobile and wireless networks world thanks to its flexible, secure, and performing characteristics. Lately, we have witnessed the increasing use of it to make more performing the deployment of machine learning (ML) techniques such as federated learning (FL). FL was debuted to improve communication efficiency compared to conventional distributed machine learning (ML). The original FL assumes a central aggregation server to aggregate locally optimized parameters and might bring reliability and latency issues. In this paper, we conduct an in-depth study of strategies to replace this central server by a flying master that is dynamically selected based on the current participants and/or available resources at every FL round of optimization. Specifically, we compare different metrics to select this flying master and assess consensus algorithms to perform the selection. Our results demonstrate a significant reduction of runtime using our flying master FL framework compared to the original FL from measurements results conducted in our EdgeAI testbed and over real 5G networks using an operational edge testbed.

==> expriments1.tex <==
\section{Numerical Evaluations}
We evaluate our framework with different settings of master node selection criteria and algorithms, also including the original central aggregation server setting, using our Edge AI and 5G Edge testbeds described in Section~\ref{sec:prelim}.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.9\linewidth]{results/legend.pdf}
	\vspace{-0.15in}
\end{figure*}
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_100_1_0.001.pdf}
		\caption{$K = 1$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_100_5_0.001.pdf}
		\caption{$K = 5$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_100_10_0.001.pdf}
		\caption{$K = 10$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_100_50_0.001.pdf}
		\caption{$K = 50$}
	\end{subfigure}
	%\vspace{-0.2in}
	\caption{Wall-clock time vs. number of rounds for $N = 100$ and 2 types of devices in the network.}
	\label{fig:N100_d2}
	\vspace{-0.12in}
\end{figure*}
\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_1000_1_0.001.pdf}
		\caption{$K = 1$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_1000_5_0.001.pdf}
		\caption{$K = 5$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_1000_10_0.001.pdf}
		\caption{$K = 10$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/2_devices/test_1000_50_0.001.pdf}
		\caption{$K = 50$}
	\end{subfigure}
	%\vspace{-0.2in}
	\caption{Wall-clock time vs. number of rounds for $N = 1000$ and 2 types of devices in the network.}
	\label{fig:N1000_d2}
	\vspace{-0.12in}
\end{figure*}
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_100_1_0.001.pdf}
		\caption{$K = 1$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_100_5_0.001.pdf}
		\caption{$K = 5$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_100_10_0.001.pdf}
		\caption{$K = 10$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_100_50_0.001.pdf}
		\caption{$K = 50$}
	\end{subfigure}
	%\vspace{-0.1in}
	\caption{Wall-clock time vs. number of rounds for $N = 100$ and 4 types of devices in the network.}
	\label{fig:N100_d4}
	\vspace{-0.12in}
\end{figure*}
\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_1000_1_0.001.pdf}
		\caption{$K = 1$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_1000_5_0.001.pdf}
		\caption{$K = 5$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_1000_10_0.001.pdf}
		\caption{$K = 10$}
	\end{subfigure}
	\hspace{-0.12in}
	\begin{subfigure}[b]{0.252\linewidth}
		\includegraphics[width=\linewidth]{results/GEV/4_devices/test_1000_50_0.001.pdf}
		\caption{$K = 50$}
	\end{subfigure}
	%\vspace{-0.2in}
	\caption{Wall-clock time vs. number of rounds for $N = 1000$ and 4 types of devices in the network.}
	\label{fig:N1000_d4}
	\vspace{-0.12in}
\end{figure*}
\subsection{Settings}
\textbf{Model setting:} For the learning task, we choose the textbook handwritten digit recognition task on MNIST dataset \cite{lecun1998gradient} with 60K training images of $28\times28$ pixels and 10 labels from 0 to 9. We consider a 2-layer neural network with sigmoid activation function in each layer and the hidden layer having size of 64. The common multi-class cross-entropy loss is applied. For local optimization, we use mini-batch SGD with batch-size of 128. Since our framework is general, the choices of model, optimization method are representative and the results apply straightforwardly to other settings.

\textbf{Network settings:} We examine various aspects of the network in use: 
\begin{itemize}
	\item Network size ranges from 100 to 1000, resembling small to moderate sized networks. The number of participants in each round is in a typical range [1,50].
	\item Device heterogeneity: Since we have 5 different types of edge AI boards, i.e., NVIDIA Jetson Nano, three generations of UP Squared Edge, Coral Dev Board (Edge TPU), we consider 2 scenarios with 2 and 4 different types of devices and each device is randomly assigned one of the available types. For each device, we also simulate different stress levels by putting workloads to occupy 25\%, 50\%, and 75\% of total resources, i.e., GPU, memory, network bandwidth. When a device participates in a round of optimization, a random stress level is drawn.
	\item Communication latency: all of our devices are placed in the same location, thus, we need to simulate the latency of transmitting model parameters between devices. To do that, we first embed all of them in a 2d plane with coordinates randomly generated in the range $[0,1000]$ and use the distance between 2 devices to measure the expected latency. Furthermore, the actual latency for an individual transmission is drawn from a distribution with mean value being the expected latency. In order to determine which distribution to use, we measure latency between devices in our 5G testbed and find the best fit distribution. We find that the Generalized Extreme Value distribution is the best. We also consider the intuitive Gaussian distribution to further increase generalization.
\end{itemize}

\subsection{Results}
We measure the time it takes to perform a number of FL rounds when each of the master node selection algorithm is used in our framework. Time is wall-clock and includes both communication and computation times. Here we only measure the time and not the performance due to the fact that with the same number of rounds, the performance would be exactly the same for all master node selection algorithms. We also include the time it takes for the optimal master node selections, denoted by \optimalk{} and \optimaln{} respectively, which essentially try every candidate node and pick the one with least amount of time at each FL round. Our results are demonstrated in Figures~\ref{fig:N100_d2}, \ref{fig:N1000_d2}, \ref{fig:N100_d4}, and \ref{fig:N1000_d4}.

\textbf{Comparison to the central server setting:} Our first observation is that the central aggregation server setting requires substantially more time than any other master node selection algorithms. For example, it takes up to 4 times more than the \optimaln{}, \stressn{}, and \pown. This difference gets larger as the number of participants in an FL round becomes smaller as the fixed server does not take into account the locations of participating devices. The group of random master node selections require marginally less time than the fixed server setting, however, they are still far from optimal for the same reason as for the fixed server.

\textbf{Comparison to the optimal selections:} The second important observation is that master selection algorithms based on least stress with gossip protocol and proof-of-work, requires mostly the same amount of time as the optimal selections, for the same number of FL rounds. Particularly, time of \stressk{} and \powk{} are similar to that of \optimalk, and \stressn{} and \pown{} are similar to \optimaln{}. This is due to the fact that both gossip algorithm and proof-of-work puzzle are very fast, i.e., a few second for a run, compared to the local optimization time. Furthermore, for $K \geq 5$, there is no visible difference in term of time consumption between the group that selects master among $K$ participants and the group that selects among all $N$ devices in the network.

\textbf{Comparison between different experimental settings:} We also observe an interesting pattern the number of participants $K$ becomes larger that the difference gap between the least and most time-consuming approaches gets smaller. This pattern is intuitive following the law of large number since participants are drawn randomly in the network. On another axis, as the size of network $N$ grows from 100 to 1000, the time each approach takes to perform the same number of FL rounds gets smaller, which is possibly due to denser network and, thus, distance between 2 random devices is lesser. One last thing to note is when the number of device types increases from 2 (Figures~\ref{fig:N100_d2}, \ref{fig:N1000_d2}) to 4 - more diverse environment (Figures~\ref{fig:N100_d4}, \ref{fig:N1000_d4}), all the curves exhibit smooth increment of time as the optimization progresses.

==> intro1.tex <==
\section{Introduction}
Running tasks or applications at the network edge becomes more attractive as the edge is pervasive, and everything cannot be run in the cloud due to latency, reliability, bandwidth, or privacy issues. 
In the last decade, internet of things (IoT), such as sensors that measure temperature, humidity, light, etc., become very inexpensive and have been plugged into Raspberry Pi or Arduino type devices for innovative works. Likewise, machine learning (ML) technology is at the same stage now. For instance, Google TensorFlow unit, which is similar in size from typical Raspberry Pi or Arduino type devices, is a very similar unit to what one sees in the Google Cloud. Its coral version is smaller than penny, which is an ML accelerator. The ML hardware is now becoming easier to embed in the edge systems. 
ML software, such as tiny ML, is coming as well to shrink a deep learning network to fit on edge hardware in addition to standard practice, such as feature reduction. Moreover, architectures one benefits from the cloud -- not just processors, but the ideas of containerization, such as Kubernetes -- are coming to the edge TensorFlow light as their IoT edge. As all these things that are now extensions of the cloud are maturing and moving southbound towards the edge, ML will be a reality at the edge.

Federated learning (FL) \cite{mcmahan2017communication,li2020federated,mcmahan2021advances,konevcny2016federated} is recently introduced as a prime ML framework for learning on the edge, on local devices without sharing private data, while still benefiting from the massive and diverse available data from the federation of devices in the network as a typical decentralized ML. Thus, FL offers appealing features including fundamental data privacy protection, communication efficiency, and decentralized learning.With the growing concern regarding data privacy, tech giants like Google and Facebook are exerting immense efforts in developing software and hardware support.

The principal design of FL includes a network of devices, that are capable of training an ML model on the local data, and a central aggregation server, that routinely aggregates local models from a small set of devices to form a global model to distribute for the entire network. This centralized aggregation server poses some major issues as it is the central point of failure. On one hand, if the server is unavailable due to networking problem, e.g., under cyber attack, power failure, the learning process stops and even needs to restart all over. On the other hand, the communication cost may be extremely high in practical applications on the entire Internet.

In this paper, we introduce a more communication-efficient FL framework to address the cumbersome centralized server setting. Earlier efforts in this direction \cite{kim2019blockchained,qu2020decentralized} employ blockchain to remove the server component, however, the employment of blockchain introduces extensive communication cost and delay due to its characteristics, rendering this approach likely unsuitable for many applications. Our main idea is to dynamically select the best \emph{flying master} node to perform model aggregation either among the participants or entire network at every round of FL optimization. This flying master node is optimized based on communication cost with respect to the particular set of participants in that round and available computing resources. Thus, it will provide much lower delay for both communication and aggregation. To pick the master node, we investigate consensus algorithms using a specified metric, termed \emph{Stress}, measuring the suitability of each candidate node. We propose to use Gossip and proof-of-work consensus algorithms and perform extensive experiments on a real-world deployment of EdgeAI and 5G Edge Testbeds to demonstrate the better efficiency of our idea in practice.

\textcolor{red}{Possibly more result details if space allows.}

==> preliminary1.tex <==
\section{Preliminaries}
\label{sec:prelim}
We describe the canonical FL setting with a fixed server for aggregations of local models and the testbeds, i.e., EdgeAI and 5G Edge, that we built to test our approach along with the default centralized aggregation server setting.

\subsection{Federated learning setting}
In FL setting, we have a network of $N$ devices, indexed from 1 to $N$, device $i$ possesses a local dataset $\mathcal{D}_i$ that can be used to optimize a machine learning model locally. We wish to learn a model $M$ with parameter set $\mathbf{w}$ using the available data in all the devices in a distributed manner without any device sharing its data. Hence, the optimization problem is defined as follows:
\begin{align}
	\min_{\mathbf{w}} f(w) = \min_{\mathbf{w}} \frac{1}{N} \sum_{k = 1}^{N} f_k(\mathbf{w}),
\end{align}
where $f(w)$ and $f_i(w)$ are global and local cost functions. The local cost $f_k(\mathbf{w})$ depends on its local dataset $\mathcal{D}_k$, e.g.,
\begin{align}
	f_k(\mathbf{w}) = \sum_{(x,y) \in \mathcal{D}_k} f_k(\mathbf{w}, (x,y)),
\end{align}
where $(x,y)$ is a local data point.

In the original FL setting, there is a central server $\s{}$ in the network to perform aggregation of local models, i.e., aggregating locally updated parameters from a set of devices. A typical FL algorithm unrolls in $T$ rounds of communication and computation as described in Algorithm~\ref{alg:typical_fl}.
\begin{algorithm}
	\caption{FL algorithm with a central aggregation server}
	\label{alg:typical_fl}
	\hspace*{\algorithmicindent} \textbf{Input:} Number of participants $K$, number of rounds $T$\\
	\hspace*{\algorithmicindent} \textbf{Output:} Optimized model parameters $\mathbf{w}^T$
	\begin{algorithmic}[1] % The number tells where the line numbering should start
		\State Initialize $\mathbf{w}^0$
		\For{$t = 0, \dots, T-1$}
			\State $\s{}$ samples a set $\mathcal{S}_t$ of $K$ devices
			\State $\mathbf{w}^{t+1} = $ \texttt{FL\_ROUND($\s, \mathbf{w}^t, \mathcal{S}_t$)}
		\EndFor
		\Procedure{\texttt{FL\_ROUND}}{$\s$, $\mathbf{w}, \mathcal{S}$}:
%			\For{$t = 0, \dots, T-1$}
%				\State \s{} samples a set $\mathcal{S}_t$ of $K$ devices
				\State $\s{}$ sends $\mathbf{w}$ to all devices $k \in \mathcal{S}$
				\State Each device $k \in \mathcal{S}$ performs local optimization from $\mathbf{w}$ to obtain $\mathbf{w}'_k$ using its dataset $\mathcal{D}_k$
				\State Each device $k \in \mathcal{S}$ sends $\mathbf{w}'_k$ back to $\s{}$
				\State $\s{}$ aggregates $\mathbf{w}'_k, \forall k \in \mathcal{S}$ to form $\mathbf{w}'$
				\State \Return $\mathbf{w}'$
%			\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
In round $t$, the central server first selects a small set $\mathcal{S}_t$ of $K$ devices and distributes the current model $\mathbf{w}^t$ to those selected devices (Lines~1-2). Then, each selected device performs local optimization, e.g., commonly SGD, starting from the received model parameters $\mathbf{w}^t$ and produces an updated parameter set $\mathbf{w}_k^{t+1}$. These parameters $\mathbf{w}_k^{t+1}, \forall k \in \mathcal{S}_t$ are sent back to the central server to be aggregated and form a new model with parameter set $\mathbf{w}^{t+1}$.

A good example of FL algorithm is \fedavg \cite{mcmahan2017communication}, which is the first to propose FL and creates an enormous amount of follow-up works on this problem. \fedavg{} uses uniform sampling to select a set of participants in each round and employs a small number of SGD steps for local optimization. Importantly, \fedavg{} performs exceptionally well, requiring only a small number of participants in each round, e.g., $K = 10$, in a network of thousand devices in comparison to the case where all the data are located in a single machine and accessible.

\subsection{EdgeAI and 5G Edge Testbeds}
In our EdgeAI testbed (Fig.\ref{fig:edgeai}), we introduce edge devices' heterogeneity by using three distinct types of AI accelerators, such as Intel Movidius Myriad X VPU, Google Edge TPU, NVIDIA 128-core Maxwell GPU. The three system-on-chip are hosted respectively in three different Single-Board Computers (SBCs): UP Squared AI Edge, Coral Dev Board, and NVIDIA Jetson Nano. Fig.\ref{fig:edgeai_hw} summarizes the other hardware characteristics of the devices. It can be noticed how the SBCs have heterogeneous features also from CPU, memory RAM, and storage perspective.

\begin{figure}
\includegraphics[width=8.5cm]{Figures/edgeai_tesbed.pdf}
\centering
\caption{EdgeAI testbed setup.}
\label{fig:edgeai}
\end{figure}
\vspace{1\baselineskip}
%\textcolor{red}{Detailed descriptions go here with possibly demo picture.}

\begin{figure}
\includegraphics[width=8.5cm]{Figures/hw_features.png}
\centering
\caption{EdgeAI testbed devices' hardware features.}
\label{fig:edgeai_hw}
\end{figure}
\vspace{1\baselineskip}
